Localized Symbolic Knowledge Distillation for Visual Commonsense Models

Instruction following vision-language (VL) models offer a flexible interface that supports a broad range of multimodal tasks in a zero-shot fashion. However, interfaces that operate on full images do not directly enable the user to "point to" and access specific regions within images. This capability is important not only to support reference-grounded VL benchmarks, but also, for practical applications that require precise within-image reasoning. We build Localized Visual Commonsense models, which allow users to specify (multiple) regions as input. We train our model by sampling localized commonsense knowledge from a large language model (LLM): specifically, we prompt an LLM to collect commonsense knowledge given a global literal image description and a local literal region description automatically generated by a set of VL models. With a separately trained critic model that selects high-quality examples, we find that training on the localized commonsense corpus can successfully distill existing VL models to support a reference-as-input interface. Empirical results and human evaluations in a zero-shot setup demonstrate that our distillation method results in more precise VL models of reasoning compared to a baseline of passing a generated referring expression to an LLM.

==> figures/filtering_human_eval.tex <==
\begin{table}[t]
\normalsize
\centering
\scalebox{0.45}{
\begin{tabular}{l| c c }
\toprule

& \textbf{With Filtering} & \textbf{Without Filtering} \\
\midrule
{\textbf{QA Correctness}} & $2.41  \pm 0.74$ & $1.97 \pm 0.84$ \\
{\textbf{Rationale Justificaiton}} & $2.34 \pm 0.82$ & $1.87 \pm 0.87 $ \\ 
\end{tabular}
}
\caption {
Human ratings of corpus with and without filtering. We ask 3 human annotators to rate the instances in a Likert scale (1 to 3) and calculate the average ratings.
}  
\label{tab:filtering_human_eval}
\vspace{0.5mm}
%\end{center}
\end {table}


==> tables/vcr_x.tex <==
\begin{table}[t]
\normalsize
\centering
\scalebox{0.8}{
\begin{tabular}{l| c c | c c c c c | c c c | c}
\toprule

 & \multicolumn{2}{c}{\textbf{VCR Q $\rightarrow$ A}} & 
 \multicolumn{5}{c}{\textbf{N-Gram Scores}}
 \multicolumn{4}{c}{\textbf{e-VIL}} 
\\ 

\textbf{Approach} & Multiple Choice & BS & B-4 & R & M & C & S & $S_O$ & $S_T$ & $S_E$ & BS\\
\midrule 
% &  & 30K & In-Domain & & & \\
 e-UG  & - & - & 4.3 & 22.5 & 11.8 & 32.7 & 12.6 & 19.3 & 69.8 & 27.6 & 79.0 \\
 NLX-GPT & - & - & 6.6 & 26.4 & 12.2 & 46.9 &  18.8 & - & - & - &  80.3 \\
 OFA-X & - & - & 6.1 & 25.1 & 12.2 & 48.5 & 18.8 & - & - & - &  79.8\\
 UMAE & 56.7 & 86.0 & 13.4 & 29.5 & 17.5 & 47.3 & 26.5 & 22.8 & 56.7 & 40.3 & 81.9 \\
 BLIP-2 (FlanT5-XL) & 53.0 \\
 BLIP-2 (FlanT5-XXL) & 50.6 \\
 BLIP-2 (FlanT5-XXL) MMSymKD & 56.2\\
 \bottomrule
\end{tabular}
}
\caption {
VCR-X Finetuning Performance. We report the Q $\rightarrow$ A accuracy measured by model perplexity. N-Gram and Bert scores (BS) are reported. Following UMAE, $S_T$ is the task ($Q \rightarrow A$) accuracy based on perplexity, $S_E$ is the harmonic mean of N-Gram scores, and $S_O$ is the product of $S_T$ and $S_E$. For BLIP-2, nucleus sampling of $p=0.9$ is used. 
}
\label{tab:vcr-x}
\vspace{1.5mm}
%\end{center}
\end {table}
